Trust-based Multiagent Consensus or Weightings Aggregation

We introduce a framework for reaching a consensus amongst several agents communicating via a trust network on conflicting information about their environment. We formalise our approach and provide an empirical and theoretical analysis of its properties.

==> data.tex <==










